Open-MAGVIT2: An Open-Source Project Toward Democratizing Auto-regressive Visual Generation

The Open-MAGVIT2 project produces an open-source replication of Google's MAGVIT-v2 tokenizer, a tokenizer with a super-large codebook (i.e., $2^{18}$ codes), and achieves the state-of-the-art reconstruction performance on ImageNet and UCF benchmarks. We also provide a tokenizer pre-trained on large-scale data, significantly outperforming Cosmos on zero-shot benchmarks (1.93 vs. 0.78 rFID on ImageNet original resolution). Furthermore, we explore its application in plain auto-regressive models to validate scalability properties, producing a family of auto-regressive image generation models ranging from 300M to 1.5B. To assist auto-regressive models in predicting with a super-large vocabulary, we factorize it into two sub-vocabulary of different sizes by asymmetric token factorization, and further introduce ``next sub-token prediction'' to enhance sub-token interaction for better generation quality. We release all models and codes to foster innovation and creativity in the field of auto-regressive visual generation.

==> table/reconstruction.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{4pt}
    \renewcommand\arraystretch{1.1}
    \caption{Reconstruction performance of different tokenizers on $256 \times 256$
 ImageNet 50k validation set. Open-MAGVIT2 achieves SOTA results on different downsampling rates. $\dagger$ specifies that the training is on OpenImages. $*$ denotes that the results are from the direct inference using the model trained with $128 \times 128$ resolution without fine-tuning.}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{lcccccccc}
        \toprule
        \multirow{2}{*}{\textbf{Method}} & \textbf{Token} & \multirow{2}{*}{\textbf{Tokens}} & \multirow{2}{*}{\textbf{Ratio}} & \textbf{Train} & \textbf{Codebook} & \multirow{2}{*}{\textbf{rFID}$\downarrow$} & \multirow{2}{*}{\textbf{PSNR}$\uparrow$} & \textbf{Codebook} \\
        & \textbf{Type} &  & & \textbf{Resolution} & \textbf{Size} & & & \textbf{Usage}$\uparrow$ \\
        \midrule
        VQGAN~\citep{vqgan} & 2D & $16 \times 16$ & 16 & $256 \times 256$ & 1024 & 7.94 & 19.4 & $-$ \\
        SD-VQGAN~\citep{ldm} & 2D & $16 \times 16$ & 16 & $256 \times 256$ & 16384 & 5.15 & $-$ & $-$ \\
        MaskGIT~\citep{maskgit} & 2D & $16 \times 16$ & 16 & $256 \times 256$ & 1024 & 2.28 & $-$ & $-$ \\
        LlamaGen~\citep{llamagen} & 2D & $16 \times 16$ & 16 & $256 \times 256$ & 16384 & 2.19 & 20.79 & 97\% \\
        \textbf{Open-MAGVIT2} & 2D & $16 \times 16$ & 16 &$256 \times 256$ & 262144 & \textbf{1.17} & \textbf{22.64} & \textbf{100\%} \\ \hline
        ViT-VQGAN~\citep{vit-vqgan} & 2D & $32 \times 32$ & 8 & $256 \times 256$ & 8192 & 1.28 & $-$ & $-$ \\
        VQGAN$^{\dagger}$~\citep{vqgan} & 2D & $32 \times 32$ & 8 & $256 \times 256$ & 16384 & 1.19 & 23.38 & $-$ \\
        SD-VQGAN$^{\dagger}$~\citep{ldm} & 2D & $32 \times 32$ & 8 & $256 \times 256$ &  16384 & 1.14 & $-$ & $-$ \\
        OmiTokenizer-VQ~\citep{omnitokenizer} & 2D & $32 \times 32$ & 8 & $256 \times 256$ & 8192 & 1.11 & $-$ & $-$ \\
        LlamaGen~\citep{llamagen} & 2D & $32 \times 32$ & 8 & $256 \times 256$ & 16384 & 0.59 & 24.45 & $-$ \\
        \textbf{Open-MAGVIT2}$^{*}$ & 2D & $32 \times 32$ & 8 &$128 \times 128$ & 262144 & \textbf{0.34} & \textbf{27.02} & \textbf{100\%} \\ \hline
        Titok-L~\citep{titok} & 1D & 32 & $-$ & $256 \times 256$ & 4096 & 2.21 & $-$ & $-$ \\
        Titok-B~\citep{titok} & 1D & 64 & $-$ & $256 \times 256$ & 4096 & 1.70 & $-$ & $-$ \\
        Titok-S~\citep{titok} & 1D & 128 & $-$ & $256 \times 256$ & 4096 & 1.71 & $-$ & $-$ \\
    \bottomrule
    \end{tabular}}
    \label{tab:recon1}
\end{table}

==> table/release_model.tex <==
\begin{table}
    \centering
    \setlength{\tabcolsep}{3pt}
    \renewcommand\arraystretch{1.0}
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Method}  & \textbf{Parameters} & \textbf{Data} & \textbf{Tokens} &  \textbf{FID}\\
    \midrule
    \multicolumn{5}{c}{\textit{VQ-VAE}} \\
    \midrule
    Open-MAGVIT2-Tokenizer & 115M & $128 \times 128$ Imagenet & $16\times 16$ & $1.18$ \\
    Open-MAGVIT2-Tokenizer & 115M & $256 \times 256$ Imagenet & $16\times 16$ & $1.17$ \\
    \midrule
    \multicolumn{5}{c}{\textit{Auto-Regressive Transformer}} \\
    \midrule
    Open-MAGVIT2-B & 337M & $256 \times 256$ Imagenet & $16 \times 16$ & $-$ \\
    Open-MAGVIT2-L & 779M & $256 \times 256$ Imagenet & $16 \times 16$ & $-$ \\
    Open-MAGVIT2-XL & 1.5B & $256 \times 256$ Imagenet & $16 \times 16$ & $-$ \\
    \bottomrule
    \end{tabular}}
    \caption{\textbf{Released version of Open-MAGVIT2}.}
    \label{tab:released}
\end{table}
